Belief Space Planning for Mobile Robots with Range Sensors using iLQG

In this work, we use iterative Linear Quadratic Gaussian (iLQG) to plan motions for a mobile robot with range sensors in belief space. We address two limitations that prevent applications of iLQG to the considered robotic system. First, iLQG assumes a differentiable measurement model, which is not true for range sensors. We show that iLQG only requires the differentiability of the belief dynamics. We propose to use a derivative-free filter to approximate the belief dynamics, which does not require explicit differentiability of the measurement model. Second, informative measurements from a range sensor are sparse. Uninformative measurements produce trivial gradient information, which prevent iLQG optimization from converging to a local minimum. We densify the informative measurements by introducing additional parameters in the measurement model. The parameters are iteratively updated in the optimization to ensure convergence to the true measurement model of a range sensor. We show the effectiveness of the proposed modifications through an ablation study. We also apply the proposed method in simulations of large scale real world environments, which show superior performance comparing to the state-of-the-art methods that either assume the separation principle or maximum likelihood measurements.

==> tex/ilqg_formulations.tex <==
\section{}
\label{sec: iLQG formulation details}
In this section, we provide the detailed formulations of iLQG as a supplementary of Sec.~\ref{sec: preliminary}.
Assume the availability of a nominal trajectory, $\crl{\bar{\bm{b}}_0, \bar{\bm{u}}_0, \bar{\bm{b}}_1, \bar{\bm{u}}_1, \dots, \bar{\bm{b}}_l}$.
The nonlinear optimization problem in~\eqref{eq: objective function} is converted to LQG starting from approximating the value function of the last step,
\small
\begin{gather*}
  V_l^*\prl{\bm{b}_l} \approx \frac{1}{2} \tilde{\bm{b}}_l^\top S_l \tilde{\bm{b}}_l + \bm{s}_l \tilde{\bm{b}}_l + s_l,\\
  S_l = \frac{\partial^2 c_l}{\partial \bm{b}^2}(\bar{\bm{b}}_l),\;
  \bm{s}_l = \frac{\partial c_l}{\partial \bm{b}}(\bar{\bm{b}}_l), \;
  s_l = c_l(\bar{\bm{b}}_l).
\end{gather*}
\normalsize
where $\tilde{\bm{b}} = \bm{b} - \bar{\bm{b}}$ is the belief error.
Similarly, we use $\tilde{\bm{u}} = \bm{u} - \bar{\bm{u}}$ in the following to represent the control error.
The value functions and control policies for the remaining time steps are computed recursively as follows.

At time step $t$, the value function and control policy is obtained by solving the following optimization,
\begin{equation*}
  V_t^*\prl{\bm{b}_t} = \min_{\bm{u}_t} \Big\{
                      c_t(\bm{b}_t, \bm{u}_t) +
                      \underset{\bm{w}_{t+1}}{\mathbb{E}}\big\{ V_{t+1}^*\prl{\Phi\prl{\bm{b}_t, \bm{u}_t, \bm{w}_{t+1}}} \big\}
                      \Big\}
\end{equation*}
With some abuse of notation, the innovation noise $\bm{w}_{t+1}$ is used in the belief dynamics $\Phi(\cdot)$,~\eqref{eq: general belief dynamics}, to replace $\bm{z}_{t+1}$.
Differentiating $\Phi(\bm{b}_t, \bm{u}_t, \bm{w}_{t+1})$ and $c_t(\bm{b}_t, \bm{u}_t)$ to the first and second order around $\bm{b}_t=\bar{\bm{b}}_t$, $\bm{u}_t=\bar{\bm{u}}_t$, and $\bm{w}_{t+1}=\bm{0}$ gives,
\small
\begin{gather*}
  % Quadratize ct().
  \begin{aligned}
    &Q_t = \frac{\partial^2 c_t}{\partial \bm{b}_t^2}, &
    &R_t = \frac{\partial^2 c_t}{\partial \bm{u}_t^2}, &
    &P_t = \frac{\partial^2 c_t}{\partial \bm{u}_t \partial \bm{b}_t}, \\
    &\bm{q}_t = \frac{\partial c_t}{\partial \bm{b}_t}, &
    &\bm{r}_t = \frac{\partial c_t}{\partial \bm{u}_t}, &
    &p_t = c_t\prl{\bar{\bm{b}}_t, \bar{\bm{u}}_t}, \\
  \end{aligned} \\
  % Linearize Phi().
  \begin{aligned}
    &F_t = \frac{\partial \Phi}{\partial \bm{b}_t}, &
    &G_t = \frac{\partial \Phi}{\partial \bm{u}_t}, &
    &W_t = \frac{\partial \Phi}{\partial \bm{w}_{t+1}}, \\
    &\bm{e}_t^i = W_t^{(i)}, &
    &F_t^i = \frac{\partial W_t^{(i)}}{\partial \bm{b}_t}, &
    &G_t^i = \frac{\partial W_t^{(i)}}{\partial \bm{u}_t},
  \end{aligned}
\end{gather*}
\normalsize
where $W_t^{(i)}$ represents the $i$\textsuperscript{th} column of $W_t$.
Then, $V_t(\cdot)$ can be approximated by a quadratic function,
\small
\begin{equation}
  \label{eq: approximation for the value function at time step t}
  V_t^*\prl{\bm{b}_t} \approx \min_{\bm{u}_t} \Big\{
                            \frac{1}{2} \begin{pmatrix}\tilde{\bm{b}}_t \\ \tilde{\bm{u}}_t \end{pmatrix}^\top
                                        \begin{pmatrix}C_t & E_t^\top \\ E_t & D_t \end{pmatrix}
                                        \begin{pmatrix}\tilde{\bm{b}}_t \\ \tilde{\bm{u}}_t \end{pmatrix}  +
                            \begin{pmatrix}\bm{c}_t & \bm{d}_t\end{pmatrix}
                            \begin{pmatrix}\tilde{\bm{b}}_t \\ \tilde{\bm{u}}_t \end{pmatrix} +
                            e_t
                            \Big\}
\end{equation}
\normalsize
where,
\small
\begin{align*}
  C_t &= Q_t + F_t^\top S_{t+1} F_t + \sum_{i=1}^n F_t^{i\top} S_{t+1} F_t^i,\\
  D_t &= R_t + G_t^\top S_{t+1} G_t + \sum_{i=1}^n G_t^{i\top} S_{t+1} G_t^i,\\
  E_t &= P_t + G_t^\top S_{t+1} F_t + \sum_{i=1}^n G_t^{i\top} S_{t+1} F_t^i,\\
  \bm{c}_t &= \bm{q}_t + \bm{s}_{t+1}F_t + \sum_{i=1}^n \bm{e}_t^{i\top} S_{t+1} F_t^i,\\
  \bm{d}_t &= \bm{r}_t + \bm{s}_{t+1}G_t + \sum_{i=1}^n \bm{e}_t^{i\top} S_{t+1} G_t^i,\\
  e_t &= p_t + s_{t+1} + \frac{1}{2}\sum_{i=1}^n \bm{e}_t^{i\top} S_{t+1} \bm{e}_t^i.
\end{align*}
\normalsize
Solving the quadratic program in~\eqref{eq: approximation for the value function at time step t} produces the feedback control policy at time step $t$,
\begin{equation}
  \label{eq: feedback policy at time step t}
  \tilde{\bm{u}}_t = -D_t^{-1} E_t \tilde{\bm{b}}_t - D_t^{-1}\bm{d}_t^\top,
\end{equation}
and,
\small
\begin{align*}
  &V_t^*\prl{\bm{b}_t} \approx \frac{1}{2}\tilde{\bm{b}}_t^\top S_{t} \tilde{\bm{b}}_t + \bm{s}_t \tilde{\bm{b}}_t + s_t, \\
  &S_t = C_t - E_t^\top D_t^{-1} E_t, \\
  &\bm{s}_t = \bm{c}_t - \bm{d}_t D_t^{-1} E_t, \\
  &s_t = e_t - \frac{1}{2} \bm{d}_t D_t^{-1} \bm{d}_t^\top.
\end{align*}
\normalsize
By proceeding to time step $0$, control polices for all time steps are obtained.
The rest steps of iLQG follow Alg.~\ref{alg: belief space iLQG}.

